When and what to learn in a changing world

A decision-maker periodically acquires information about a changing state, controlling both the timing and content of updates. I characterize optimal policies using a decomposition of the dynamic problem into optimal stopping and static information acquisition. Eventually, information acquisition either stops or follows a simple cycle in which updates occur at regular intervals to restore prescribed levels of relative certainty. This enables precise analysis of long run dynamics across environments. As fixed costs of information vanish, belief changes become lumpy: it is optimal to either wait or acquire information so as to exactly confirm the current belief until rare news prompts a sudden change. The long run solution admits a closed-form characterization in terms of the "virtual flow payoff". I highlight an illustrative application to portfolio diversification.

==> Tikz/Tikz_Portfolio_Example2/Portfolio_Example_cav.tex <==
\pgfplotsset{
        table/search path={Tikz_Portfolio_Example2},
    }

\begin{tikzpicture}
\begin{axis}[
  xmin=0, xmax=1,
  ymin=1.79, ymax=1.86,
  % y=4cm,
  % x=3cm,
  clip = false,
  height=7cm,
  width=10cm,
  % axisratio=2,
  % xtick = {0,.5,1},
  xtick distance = 1,
  ytick distance = 1,
  ticklabel style = {font=\tiny},
  % x label style = {at={(1.02,-0.1)},anchor=west,font=\small},
  % xlabel={$p$},
  ylabel={},
  axis lines=middle,
  axis line style={-},
  % legend pos= north west,
  legend style={at={(.5,.7)},anchor=west,font=\footnotesize,draw=none}
  ]

  % \addplot+ [mathematicablue, no marks, smooth] table {u.table} node[left,pos=.7] {$u$}; 
  \only<1->{\addplot+ [mathematicablue, thick, no marks, smooth] table {v_net.table} node[right,pos=.82] {$v-c$};}
  \only<3>{\addplot+ [mathematicablue, thick, dashed, no marks, smooth] table {Cav_v_net.table} node[above,pos=.5] {$\Cav[v-c]$};}
  \only<4->{
  \addplot [mathematicagreen,mark=*,only marks,mark options={color=mathematicagreen,fill=mathematicagreen}] table {targets_vnet.table};
  \addplot [mathematicagreen,mark=*,only marks,mark options={color=mathematicagreen,fill=mathematicagreen}] table {targets_vnet_axis.table};
  \addplot [mathematicagreen,no marks,very thick,dashed] table {targets1_vnet_axis.table};
  \addplot [mathematicagreen,no marks,very thick,dashed] table {targets2_vnet_axis.table};
  \addplot [mathematicagreen,no marks,very thick,dashed] table {targets3_vnet_axis.table};
  \addplot [mathematicagreen,no marks,very thick,dashed] table {targets1_vnet.table};
  \addplot [mathematicagreen,no marks,very thick,dashed] table {targets2_vnet.table};
  \addplot [mathematicagreen,no marks,very thick,dashed] table {targets3_vnet.table};
  }
  \only<5->{
  \addplot [mathematicaorange,mark=diamond*,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds1_vnet.table};
  \addplot [mathematicaorange,mark=diamond*,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds2_vnet.table};
  \addplot [mathematicaorange,mark=diamond*,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds3_vnet.table};
  \addplot [mathematicaorange,mark=diamond*,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds4_vnet.table};
  \addplot [mathematicaorange,mark=diamond*,smooth,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds1_vnet_axis.table};
  \addplot [mathematicaorange,mark=diamond*,smooth,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds2_vnet_axis.table};
  \addplot [mathematicaorange,mark=diamond*,smooth,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds3_vnet_axis.table};
  \addplot [mathematicaorange,mark=diamond*,smooth,very thick,mark options={color=mathematicaorange,fill=white}] table {thresholds4_vnet_axis.table};

  \addplot [<->, gray, dotted] coordinates {(.35,1.855)  (.35,1.846)} node[left,pos=.5] {$\kappa$};
  \addplot [<->, gray, dotted] coordinates {(.65,1.855)  (.65,1.846)} node[right,pos=.5] {$\kappa$};
  \addplot [<->, gray, dotted] coordinates {(.06,1.829)  (.06,1.821)} node[left,pos=.5] {$\kappa$};
  \addplot [<->, gray, dotted] coordinates {(.94,1.829)  (.94,1.821)} node[right,pos=.5] {$\kappa$};
  }

\end{axis}
\end{tikzpicture}


==> Tikz/Tikz_Portfolio_Example2/Portfolio_Example_cav_dynamics.tex <==
\pgfplotsset{
        table/search path={Tikz_Portfolio_Example},
    }

\begin{tikzpicture}
\begin{axis}[
  xmin=0, xmax=1,
  ymin=.165, ymax=.187,
  % y=4cm,
  % x=3cm,
  height=7cm,
  width=10cm,
  % axisratio=2,
  xtick = {0,.5,1},
  ytick distance = .1,
  ticklabel style = {font=\tiny},
  % x label style = {at={(1.02,-0.1)},anchor=west,font=\small},
  % xlabel={$p$},
  ylabel={},
  axis lines=middle,
  axis line style={-},
  % legend pos= north west,
  legend style={at={(.5,.7)},anchor=west,font=\footnotesize,draw=none}
  ]

% \addplot+ [mathematicablue, no marks, smooth] table {u.table} node[left,pos=.7] {$u$}; 
\addplot+ [mathematicaorange, thick, no marks, smooth] table {v_net1.table} node[right,pos=.8] {$v-c$};
\addplot+ [mathematicaorange, thick, dashed, no marks, smooth] table {Cav_v_net1.table} node[below,pos=.5] {$\Cav[v-c]$};

\addplot [mathematicagreen,mark=*,only marks,mark options={color=mathematicagreen,fill=mathematicagreen}] table {targets1_vnet.table};
\addplot [mathematicagreen,mark=*,only marks,mark options={color=mathematicagreen,fill=mathematicagreen}] table {targets1_vnet_axis.table};

\addplot [mathematicagreen,no marks,thick,dashed] table {targets1_vnet_axis.table};
\addplot [mathematicaorange,mark=diamond*,only marks,mark options={color=mathematicaorange,fill=white}] table {thresholds1_vnet_1.table};
\addplot [mathematicaorange,mark=diamond*,only marks,mark options={color=mathematicaorange,fill=white}] table {thresholds2_vnet_1.table};
\addplot [mathematicaorange,mark=diamond*,smooth,thick,mark options={color=mathematicaorange,fill=white}] table {thresholds1_vnet_axis_1.table};
\addplot [mathematicaorange,mark=diamond*,smooth,thick,mark options={color=mathematicaorange,fill=white}] table {thresholds2_vnet_axis_1.table};

\node[cross out, draw=myblue, fill=myblue, very thick, inner sep=0pt, minimum size=2pt, label=below:{\textcolor{myblue}{$\pi$}}] (pi) at (axis cs:.5,0) {};


% \addplot+ [red, dashed, no marks, smooth] table {sigmaovertwo.table};
\end{axis}
\end{tikzpicture}


==> Tikz/Tikz_Portfolio_Example2/Portfolio_Example_strats.tex <==
\pgfplotsset{
        table/search path={Tikz_Portfolio_Example},
    }
\begin{tikzpicture}
\begin{axis}[
  xmin=0, xmax=1,
  ymin=0, ymax=1.2,
  % y=2.5cm,
  % x=3cm,
  height=4cm,
  width=6cm,
  clip=false,
  % axisratio=2,
  xtick = {0,.5,1},
  ytick distance = .5,
  ticklabel style = {font=\tiny},
  % x label style = {at={(1.02,-0.1)},anchor=west,font=\small},
  % xlabel={$p$},
  ylabel={},
  axis lines=middle,
  axis line style={-},
  legend pos= north west,
  legend style={at={(1.1,.6)},anchor=west,font=\footnotesize,draw=none}
  ]

\addplot+ [mathematicaorange, thick, no marks] table {beta.table} node[above,pos=.85] {\footnotesize $\beta^*(p)$};
% \addlegendentry{$\beta^*(p)$};
\addplot+ [mathematicagreen, thick, no marks] table {gamma.table} node[right,pos=.15] {\footnotesize $\gamma^*(p)$};

% \addplot+ [red, dashed, no marks, smooth] table {riskcomponent.table} node[above,pos=.5] {\footnotesize $\frac{\alpha}{2} \sigma^*(p)$} ;
% \addlegendentry{$\gamma^*(p)$};
\end{axis}
\end{tikzpicture}


==> Tikz/Tikz_Portfolio_Example2/Portfolio_Example_u.tex <==
\pgfplotsset{
        table/search path={Tikz_Portfolio_Example2},
    }
\begin{tikzpicture}
\begin{axis}[
  xmin=0, xmax=1,
  ymin=0, ymax=10,
  % y=4cm,
  % x=3cm,
  height=6cm,
  width=10cm,
  clip=false,
  % axisratio=2,
  xtick = {0,1},
  ytick = false,
  ticklabel style = {font=\tiny},
  % x label style = {at={(1.02,-0.1)},anchor=west,font=\small},
  % xlabel={$p$},
  ylabel={},
  axis lines=middle,
  axis line style={-},
  % legend pos= north west,
  legend style={at={(.5,.7)},anchor=west,font=\footnotesize,draw=none}
  ]

\addplot+ [mathematicablue, thick, no marks, smooth] table {u.table} node[left,pos=.8] {\normalsize $u(p)$} ; 

% \draw [decorate,decoration = {brace,raise = 3.5pt,mirror}, mathematicablue] (pLstar) --  (plstar) node [pos=.5, label=below:{\textcolor{mathematicablue}{\only<1|handout:0>{$\approx \tau^0$} \only<2->{$\approx \tau^*$} }}] {} ; 

\begin{scope}[decoration={calligraphic brace,amplitude=5pt,raise=-.5pt,mirror}]
    \draw[thick,decorate,pen colour={mathematicablue},mathematicablue] (axis cs:0.4184,0) -- (axis cs:0.5816,0)
     node[midway,below=1ex]{\small safe asset};
    \draw[thick,decorate,pen colour={mathematicablue},mathematicablue] (axis cs:0.0537,0) -- (axis cs:0.4183,0)
     node[midway,below=1ex]{\small mix};
    \draw[thick,decorate,pen colour={mathematicablue},mathematicablue] (axis cs:0,0) -- (axis cs:0.0536,0)
     node[midway,below=1ex]{\small asset 0};
    \draw[thick,decorate,pen colour={mathematicablue},mathematicablue] (axis cs:0.5817,0) -- (axis cs:0.9463,0)
     node[midway,below=1ex]{\small mix}; 
     \draw[thick,decorate,pen colour={mathematicablue},mathematicablue] (axis cs:0.9464,0) -- (axis cs:1,0)
     node[midway,below=1ex]{\small asset 1}; 
    \end{scope}
% \addlegendentry{$u(p)$};

% \node[cross out, very thick, inner sep=0pt, minimum size=2pt, label=below:{\textcolor{myblue}{$\pi$}}] (pi) at (axis cs:.5,0) {};

\node[draw=mathematicablue, fill=mathematicablue, very thick, inner sep=0pt, minimum size=2pt, label=below:{}] (pAM) at (axis cs:0.0536376,0) {};
\node[draw=mathematicablue, fill=mathematicablue, very thick, inner sep=0pt, minimum size=2pt, label=below:{}] (pMS) at (axis cs:0.41835,0) {};
\node[draw=mathematicablue, fill=mathematicablue, very thick, inner sep=0pt, minimum size=2pt, label=below:{}] (pSM) at (axis cs:0.58165,0) {};
\node[draw=mathematicablue, fill=mathematicablue, very thick, inner sep=0pt, minimum size=2pt, label=below:{}] (pSM) at (axis cs:0.946362,0) {};


\end{axis}
\end{tikzpicture}


==> Tikz/Tikz_Portfolio_Example2/Portfolio_Example_value.tex <==
\pgfplotsset{
        table/search path={Tikz_Portfolio_Example2},
    }

\begin{tikzpicture}
\begin{axis}[
  xmin=0, xmax=1,
  ymin=0, ymax=1.8,
  clip=true,
  % y=4cm,
  % x=3cm,
  height=8cm,
  width=12cm,
  % axisratio=2,
  xtick = {0,1},
  ytick distance = 2,
  ticklabel style = {font=\tiny},
  % x label style = {at={(1.02,-0.1)},anchor=west,font=\small},
  % xlabel={$p$},
  ylabel={},
  axis lines=middle,
  axis line style={-},
  % legend pos= north west,
  legend style={at={(.5,.7)},anchor=west,font=\footnotesize,draw=none}
  ]

\only<1->{\addplot+ [mathematicablue, no marks, smooth] table {uoverr.table} node[left,pos=.7] {$u$}; }
\only<2->{\addplot+ [mathematicaorange, thick, no marks, smooth] table {v.table} node[left,pos=1] {$v$};}
\only<3->{\addplot+ [mathematicaorange, thick, dashed, no marks, smooth] table {GvGross.table} node[above,pos=.5] {$\mathcal{G}v$};}
% \only<5->{\addplot+ [red, thick, dotted, no marks, smooth] table {Gv.table} node[below,pos=.5] {$\mathcal{G}v-\kappa$};}
% \only<5->{
% \addplot [red,mark=diamond*,smooth,thick,mark options={color=red,fill=white}] table {thresholds1_axis.table};
% \addplot [red,mark=diamond*,smooth,thick,mark options={color=red,fill=white}] table {thresholds2_axis.table};
% \addplot [red,mark=diamond*,smooth,thick,mark options={color=red,fill=white}] table {thresholds3_axis.table};
% \addplot [red,mark=diamond*,smooth,thick,mark options={color=red,fill=white}] table {thresholds4_axis.table};
% }


% \addplot+ [red, dashed, no marks, smooth] table {sigmaovertwo.table};
\end{axis}
\end{tikzpicture}

